Robust Graph Learning Under Wasserstein Uncertainty

Graphs are playing a crucial role in different fields since they are powerful tools to unveil intrinsic relationships among signals. In many scenarios, an accurate graph structure representing signals is not available at all and that motivates people to learn a reliable graph structure directly from observed signals. However, in real life, it is inevitable that there exists uncertainty in the observed signals due to noise measurements or limited observability, which causes a reduction in reliability of the learned graph. To this end, we propose a graph learning framework using Wasserstein distributionally robust optimization (WDRO) which handles uncertainty in data by defining an uncertainty set on distributions of the observed data. Specifically, two models are developed, one of which assumes all distributions in uncertainty set are Gaussian distributions and the other one has no prior distributional assumption. Instead of using interior point method directly, we propose two algorithms to solve the corresponding models and show that our algorithms are more time-saving. In addition, we also reformulate both two models into Semi-Definite Programming (SDP), and illustrate that they are intractable in the scenario of large-scale graph. Experiments on both synthetic and real world data are carried out to validate the proposed framework, which show that our scheme can learn a reliable graph in the context of uncertainty.

==> Notation/notation.tex <==
\subsection{Notation}







 

==> RelatedWork/relatedwork.tex <==
Learning a graph topology from structured data has been a research field of concern for a long time. Historically, different literature interpret graph learning from different perspective, one of which is from statistical view. One of classical statistical model is graphical lasso   \cite{friedman2008sparse,yuan2007model,ravikumar2008model}, the general point of which is to estimate an inverse covariance matrix (also called precision matrix) from observed data. In fact, precision matrices carry the information of partial correlations between random variables. In particular, if a entry of precision matrix equals to zero, the corresponding two variables of this entry are conditional independent. Therefore, precision matrices represent the relationship between variables to a certain extent like a graph. Recently, graph signal processing has been an emerging research field \cite{shuman2013emerging, ortega2018graph}, and a variety of GSP based graph learning models are proposed. The main characteristic of GSP based models is learning a graph with some tools generalizing classical signal processing concepts, such as time-frequency analysis and filtering on graphs \cite{dong2019learning}. Under this premise, graph operators, which are foundations of GSP, such as adjacency and Laplacian matrices are the objective to learn.  The first category of noteable GSP based model is based on diffusion processes \cite{mateos2019connecting}, assuming that the observation signals are generated by applying a filtering operation to input graph signals \cite{dong2019learning}. Among diffusion-based models, stationarity assumption is one of the most studied, where eigenvalues of graph operator can be estimated using sample covariance matrix of the observed data. Then the eigenvalues are estimated with some prior knowledge of graph operators\cite{pasdeloup2017characterization, segarra2017network, egilmez2018graph}. In addition to the aforementioned stationarity assumption, dictionary-based diffusion models are also worthy of attention, where localized behavior of learned graph can be captured \cite{thanou2017learning, maretic2017graph}. In parallel with diffusion-based models, smoothness assumption also occupies an important position. Smooth signals are common in real life \cite{kalofolias2016learn, chepuri2017learning, huang2018rating}. A smoothness based learning framework was first proposed in \cite{dong2016learning} using Laplacian matrix, and \cite{kalofolias2016learn} presents a more unified framework which also includes adjacency matrices. Considering the inefficient of aforementioned model, \cite{kalofolias2018large} put forwards a large scale learning method and \cite{berger2020efficient} also improves the original smoothness-based model. 

However, none of the aforementioned models takes uncertainty into consideration. As stated in \cite{rahimian2019distributionally}, uncertainty may arise from limited observability of data and noisy measurement and can cause a non negligible difference between the learned graph and real one. Robust optimization \cite{beyer2007robust} and stochastic optimization\cite{fouskakis2002stochastic} are two common tools to cope with optimization problems with uncertainty parameters. While stochastic optimization assumes a prior distribution about unknown parameters\cite{nemirovski2009robust}, robust optimization has no distributional knowledge but minimizes the worst case costs over an uncertainty sets \cite{ben2009robust}. Distributionally robust optimization (DRO), otherwise, supposes the unknown parameters obey a certain distribution. However, only partial information of this distribution can be obtained, thus a uncertainty set on this distribution is defined. The purpose of DRO is to minimize the worst case of all distributions in uncertainty set \cite{rahimian2019distributionally, goh2010distributionally}. DRO has been applied in many fields including adversarial training\cite{staib2017distributionally}, logistic regression\cite{shafieezadeh2015distributionally}, semi-supervised learning\cite{blanchet2017semi} and \cite{gao2018robust}, etc.
    
It is worth noting that the uncertainty set in DRO is defined on distribution, hence some discrepancy metrics between probabilities need to be employed to construct an uncertainty set. In general, $\Phi$ divergence\cite{ben2013robust, duchi2016variance} and maximum mean discrepancy\cite{staib2019distributionally} are two commonly adopted metrics. Recently, Wasserstein distance has been an emerging tool to measure the discrepancy between probabilities \cite{esfahani2018data}. Wasserstein distance is originate from optimal transport theory\cite{villani2008optimal} and takes into account the geometry of the space on which the distributions are defined\cite{simou2020node2coords}. One extraordinary application of Wasserstein distance is Wasserstein generative adversarial networks\cite{arjovsky2017Wasserstein}. Due to its ability to measure the difference between two distributions, Wasserstein distance is suitable to construct uncertainty sets, which is called Wasserstein distributionally robust optimization (WDRO). Some important conclusions, such as tractable reformulations and performance guarantees, are illustrated in \cite{esfahani2018data, gao2016distributionally, blanchet2018optimal, kuhn2019Wasserstein}.

To summarize, although graph learning has become a research hot-spot for a couple of time, few of work focuses on learning a graph under uncertainty, not to mention defining the uncertainty from distributionally perspective. To the best of our knowledge, this is the first work introducing WDRO into graph learning and establishing WDRO-based learning framework under uncertainty. And due to the restriction of graph structures, WDRO-based graph learning is also different from the above-mentioned distributionally robust optimization problems, which will be demonstrated in detail in the following sections.


 
